Gamma-ray Transient Network Science Analysis Group Report

The Interplanetary Network (IPN) is a detection, localization and alert system that utilizes the arrival time of transient signals in gamma-ray detectors on spacecraft separated by planetary baselines to geometrically locate the origin of these transients. Due to the changing astrophysical landscape and the new emphasis on time domain and multi-messenger astrophysics (TDAMM) from the Pathways to Discovery in Astronomy and Astrophysics for the 2020s, this Gamma-ray Transient Network Science Analysis Group was tasked to understand the role of the IPN and high-energy monitors in this new era. The charge includes describing the science made possible with these facilities, tracing the corresponding requirements and capabilities, and highlighting where improved operations of existing instruments and the IPN would enhance TDAMM science. While this study considers the full multiwavelength and multimessenger context, the findings are specific to space-based high-energy monitors. These facilities are important both for full characterization of these transients as well as facilitating follow-up observations through discovery and localization. The full document reports a brief history of this field, followed by our detailed analyses and findings in some 68 pages, providing a holistic overview of the role of the IPN and high-energy monitors in the coming decades.

==> notes.tex <==

% \textcolor{red}{To be written last}


\textbf{comments to apply here from Bruce:}

1) "Perhaps unanticipated, the localization of gamma-ray transients has been one of the most important and productive capabilities astrophysics has ever had - playing roles in the discovery of the origin of GRBs, the first discovery of a GW source, the origin of r-process elements, the discovery of magnetars, and their soft gamma flares and giant magnetic flares, discovery of some of the most distant objects in the universe [... and continue on from here, there are many more]."

2) "The GCN has been the *key* to this productivity, the very lynchpin of modern transient multi-wavelength astrophysics. By rapidly delivering position alerts of astrophysical transients to the wider astrophysical community, the GCN leverages the instrument capability of the *entire* community, across virtually all wavelengths, and now to multi-messenger particles, an incredible "force multiplier" for NASA instruments. It has become, in effect, the point of coordination of all these assets.  [Now briefly describe how important marshalling instruments across a variety of wavelengths helped in all these landmark cases above, early IR and later opt discovery of GW170817 etc.] "

... and so here we get the readers to understand the *central* role of the GCN and subsequent versions in transient astrophysics. Not the time or place to be modest! Get NASA's attention!


3)"And so, as a central tool of astrophysics, the use and capabilities of the GTN have significant impacts on NASA's science output;  therefore strategic planning and coordination of the GTN's use and capabilities, as well as setting requirements for the instruments that feed it, are critically important to carrying out NASA's mission, including but not limited to the TDAMM requirements set forth in the decadal survey. This is particularly important in the interaction of NASA space instruments and both ground-based EM and non-EM instruments.  This report is intended to inform  NASA on how strategic planning for these capabilities and feeder instruments impacts and may improve how NASA may perform its mission."

BG says: OK, so to implement this in text, I'm proposing re-structuring the introduction following the above.  Eric's comment above is wise - let's write exec summary last.


[BG Outline Idea for executive summary: A. GTN precursors have shown that NASA can leverage astrophysics people and instrument capabilities across the entire world of astrophysics, a very powerful "force multiplier" of US NASA instrumentation expenditures, by rapidly localizing and then communicating gamma-ray transients. B. This report reviews the historical importance of NASA instrumentation localization, and leveraging of worldwide community resources, and based on this, and current decadal study mandated topics, makes recommendations for NASA actions not just on communications networks, but on full ecosystem of NASA -led discover, i.e. including recommendations on NASA instrumentation that "feeds" these networks. C. These recommendations include: i,ii,iii... ]






\vspace{10mm}
\noindent
\SL{I think the document needs to be re-ordered. It doesn't flow well in its current state.\\
To me, the IPN has two main parts:
\begin{enumerate}
    \item connecting multiple (existing) instruments
    \item launching new instrument(s) and adding them to the network
\end{enumerate}
The current document makes good arguments for both, but it hops back and forth too frequently and is hard to follow. I think it would be best to transition through the document like a timeline (past $\rightarrow$ present $\rightarrow$ future). Below is my proposed outline. If you like this idea I can rearrange the ``Science" section to reflect this.\\
\\
\textbf{----- PROPOSED OUTLINE -----}\\
\begin{enumerate}
    \item abstract
    \item executive summary
    \begin{itemize}
        \item explain what the IPN is (pros and cons)
    \end{itemize}
    \item intro
    \begin{itemize}
        \item good as is
    \end{itemize}
    \item scientific motivations
    \begin{itemize}
        \item don't organize by ``event type" organize by ``IPN function"
        \begin{itemize}
            \item 1-10 deg-sq loc
            \item promotes follow-up (which is what most facilities are designed for)
            \item good for archival/offline localizations
            \item will lead to more redshift measurements
            \item etc.
        \end{itemize}
    \end{itemize}
    \item gamma-ray transient network
    \begin{itemize}
        \item connecting the missions that already exist (i.e., working with what we have)
        \begin{itemize}
            \item real-time event-based alert stream to promote follow-up
            \item joint-mission catalogs
            \item joint-mission shared database
            \item joint-mission open source analysis software
            \item etc.
        \end{itemize}
    \end{itemize}
    \item capability requirements of future mission(s)
    \begin{itemize}
        \item where are we currently falling short and what can we do better
        \begin{itemize}
            \item super-Swift
        \end{itemize}
    \end{itemize}
    \item discussion
     \begin{itemize}
        \item this is your "actionable items" section
    \end{itemize}
    \item conclusions
    \item references
    \item appendix
     \begin{itemize}
        \item this is your "examples" section
    \end{itemize}
\end{enumerate}
}








==> past.tex <==


%EXECUTIVE SUMMARY


% The United States has played a seminal role in this field since its inception. This leadership comes through the discovery with \textit{Vela} followed by the NASA missions of \textit{Pioneer Venus Orbiter}, the \textit{Compton Gamma-ray Observatory}, the \textit{High Energy Transient Explorer 2}, to the current missions, the \textit{Neil Gehrels Swift Observatory} and \textit{Fermi}. It is also evident in the shared leadership of the InterPlanetary Network with Russia and in the Gravitational Wave-Gamma-ray Burst Working Group. Guided by scientific understand gained through these high energy monitors, the NSF supported the construction of other world-leading facilities including LIGO, IceCube, and Rubin. Together, NASA and the NSF operate a majority of the discovery facilities in time-domain and multimessenger astrophysics. 

% For multidiagnostic astronomy it is key to detect and localize events from the earliest possible signature, allowing for recovery of all possible information to better understand these events. Thus dual role elevates the importance of discovery facilities over characterization facilities, emphasizing the critical need of high energy monitors. The importance of discovery telescopes is not only scientific. Time-domain and multimessenger astrophysics is a unique tool of American soft power, with the full ecosystem requiring both international partnerships and the possibility of contributing with even amateur telescopes. Thus, positive press of local scientists working with American scientists or making use of discoveries reported by American facilities appears even in non-aligned countries, an outcome possible through very few other means. 


























%INTRO



% Perhaps unanticipated, the localization of gamma-ray transients has been one of the most important and productive capabilities in astrophysics - playing roles in the discovery of the origin of gamma-ray bursts (GRBs), the first discovery of a gravitational wave (GW) source, the origin of r-process elements, the discovery of magnetars, and their soft gamma flares and giant magnetic flares, discovery of some of the most distant objects in the universe [FIX/CHECK/FINISH ... and continue on from here]. 

% The first localization of a gamma-ray transient resulted in the discovery of cosmic gamma-ray bursts (GRBs). The Vela series of satellites, originally launched to monitor Earth for atmospheric detonations of nuclear bombs, started as a pair of spacecraft with gamma-ray detectors orbiting the Earth but on opposite sides of it.  The separation distance of $\sim10^5$\ km gives a light travel time difference of up to $\sim1$\,s. As the temporal profiles of GRBs can be measured to $\sim$\ tens of ms, this allowed for localization by drawing a timing annulus for a pair of detectors, or when the network of satellites was expanded, the intersection of the annulus for each pair of spacecraft. These multiple annuli, lead to the localization of GRB sources beyond our Solar System \citep{klebesadel1973observations}.

%Today's IPN includes virtually all gamma-ray detectors in flight, and uses multipl, intersecting annuli for localizations. The most distant [FIX/CHECK ?] member is the Konus instrument aboard the Wind spacecraft, operating since 1994 at L1. 

%The first instrument designed specifically to study gamma-ray bursts was launched on Helios-B in 1976, reaching distances of up to 2 AU. This was also the beginning of the InterPlanetary Network. This was soon joined by Pioneer Venus Orbiter and several Venera satellites with Konus instruments, allowing for the first precise localizations of gamma-ray bursts. Since then, dozens of satellites have contributed to the localization of cosmic bursts.

%Triangulation of GRBs by Vela led to the founding of the study of GRBs and identification of their astrophysical origin. The early IPN led to evidence of their cosmological origin, which was ultimately proven by BATSE onboard \textit{Compton}. The IPN led to the separation of GRBs from soft gamma-ray repeater (SGR) short bursts, following the discovery of the 1979 giant flare and repeating bursts, sometimes from supernova remnants. This ultimately led to the discovery of magnetars. The modern IPN has led to the discovery of ultra-long GRBs and the identification of extragalactic magnetar giant flares. The IPN provided initial localizations for GRB\,230307A which currently appears to have enabled the first infrared spectrum of r-process nucleosynthesis. 

%For a time, purpose-built GRB instruments were launched on planetary and solar spacecraft, e.g. the GRB experiment on-board the Ulysses spacecraft. This has not occurred in decades. The IPN operates by utilizing neutron or gamma-ray spectrometers built for study of planetary bodies, often limiting timing precision to the resolution of the data. The launch of partial coding masks, particularly the Burst Alert Telescope (BAT) on-board the \textit{Neil Gehrels Swift Observatory} (\textit{Swift}) enabled rapid reporting of localizations with uncertainty of a few arcminutes. In nearly 20 years of observing the BAT has recovered more than 1,000 GRB afterglows. While the IPN can achieve comparable localizations for very bright bursts, these take days to obtain the full data. Therefore, the importance of IPN faded.

% The contributions of NASA's Great Observatory class \textit{Compton} mission (CGRO), the heaviest payload ever launched at the time (1991), with four different gamma sensitive instruments, are extremely important. Here we point out, however, that  none of its instruments could localize sources to better than ~ few degree scale. The instruments of the much smaller 480 kg Italian-Dutch BeppoSAX spacecraft however, launched 1996,  could localize GRBs to arcminutes, and led to one of the greatest scientific "scoops" of all time: the association of long-type GRBs to events at cosmological distances. The localization of GRB970228 to 3-5 arcminutes by the WFC coded-mask aperture instrument allowed the discovery of a fading optical source near a galaxy ([FIX need reference, but got this from https://arxiv.org/pdf/1902.06119.pdf ]). ROSAT played an important part here in narrowing the position of the fading GRB afterglow to a few tens of arcsec, leaving little doubt that the optical afterglow was the same event. Soon this was followed by 970508, and absorption lines in the optical spectrum showed the source $z$ to be 0.835, the turning point in understanding GRBs as beamed emission visible from extreme redshifts. The critical lessons of this phase of gamma-ray transient history are first, the value of gamma-ray localization within a reasonable scale (here $\sim$ arcmin) for search by other, e.g. optical instruments; secondly, the great value of combining multi-wave instrumentation, here X-ray and optical, in addition to the initial gamma-ray localization. Gamma-ray instruments are much, much more productive when designed to work in concert with instruments at other wavelengths. 




% [FIX/CHECK BG says he will provide a para on the role of GCN in GW170817]

% [FIX/CHECK BG says he will provide a para on the role of GCN in the FRB in SGR1935]

%Since the launch of \textit{Fermi} in 2008 the capability of GRB monitors has remained relatively stable. In contrast, vast advances in other fields have brought new import to the use of GRB monitors. The discovery of astrophysical high-energy neutrinos in 2012 \citep{icecube2013evidence}, the proof of a high rate of fast radio bursts in 2013 \citep{thornton2013population}, the direct detection of gravitational waves in 2015 \citep{abbott2016observation}, the advancement of wide-field optical telescopes (e.g. first light in the Zwicky Transient Facility in 2017), the recovery of GRBs to very high energies beginning in 2019 \citep{2019Natur.575..455M} are a few examples. This decade there are the continued upgrades to the ground-based gravitational wave interferometers and the high energy neutrino telescopes. There are enormous capability jumps with forthcoming megaton-scale MeV neutrino detectors. There are continued advances across the electromagnetic spectrum, from Rubin to the Square Kilometer Array to the Cherenkov Telescope Array.

%The InterPlanetary Network was initiated by Kevin Hurley and was led by him until his passing late in 2021. We are now in the 50th year since the announcement of GRBs. This report seeks to answer the question of what, if anything, should be done to continue or expand the IPN. We begin with a summary of the science that is possible using prompt GRB monitors. This is followed by requests for specific outputs from the community, and commentary on how this can best be met with existing. We close with a discussion on the needs of future facilities. \textcolor{red}{hit specific section references}

% [FIX/CHECK BG says Now we need a brief paragraph connecting GCN to HAWC/AMON ICE CUBE MM instruments. ]

% During the \textit{Swift} era, the GCN has been the key to the many discoveries above, the very lynchpin of modern transient multi-wavelength astrophysics. By rapidly delivering gamma-ray transient localizations to the wider astrophysical community, the GCN leverages the instrument capability of the *entire* community, across virtually all wavelengths, and now to multi-messenger particles, an incredible "force multiplier" for NASA instruments. It has become, in effect, the point of coordination of all these assets. A GW detection of a NS-NS event by itself would be interesting, the association with a short-GRB is a big step scientifically, but the rapid dissemination of the coordinates of the event is what led to IR spectroscopy identifying the r-process elements, and it was also important in identifying the event with a kilonova of a NS in a nearby galaxy. The GTN and its antecedants are a central tool of astrophysics, and the use and capabilities of the GTN have significant impacts on NASA's science output. Therefore strategic planning and coordination of the GTN's use and capabilities, as well as setting requirements for the instruments that feed it, are critically important to carrying out NASA's mission, including but not limited to the TDAMM requirements set forth in the decadal survey. This is particularly important in the interaction of NASA space instruments and both ground-based EM and non-EM instruments.  This report is intended to inform  NASA on how strategic planning for these capabilities and feeder instruments impacts and may improve how NASA may perform its mission."






%Collapsar VHE



% \hf{This needs to be rewritten, but some thoughts regarding requirements for VHE follow-up of GRB alerts. I'm focusing here on CTA.

% My main point is that while generally we'd like to have alerts within tens of seconds to catch the prompt emission, accurate localization reported at a later time is still useful for the VHE follow up community for two reasons. First, observations of the afterglow - there's a GRB that HESS detected 10-12h after the burst, and CTA might find emission even later. Second, to reduce the number of trials in the data analysis, which will increase the detection significance or make upper limits more constraining. For the former, we're looking at localization within a few degrees within a day or so. For the latter,  anything down to 0.05 deg within say a week or month can be useful. 



% According to \url{https://arxiv.org/pdf/1709.07997.pdf}, LSTs will have a goal slewing time of 20s from anywhere in the sky (requirement: 50s). I haven't found newer numbers or anything for the MSTs. In any case, \textbf{to fully utilize CTA's slewing capabilities and have a chance to catch prompt emission from LGRBs, alerts should come in at time scales shorter than or comparable to the slewing time, so preferable less than a minute after the burst. Later time localizations are still useful to observe the afterglow.}

% In addition to the MAGIC detection, we need to mention the H.E.S.S. observation of afterglow emission 10-12 h after GRB 180720B: \url{https://www.nature.com/articles/s41586-019-1743-9}, which further constrain the emission mechanisms and (in this case, they favor SSC origin of the TeV emission as pure synchrotron would require a late-time Lorentz factor of 1000 or so, at odds with expectation. This measurement shows that \textbf{late-time GRB follow-up observations by CTA are feasible and useful (and can be greatly improved by degree-scale localization uncertainty, even if they arrive hours or even a day after the burst).}

% }

% \eb{Can place the LHAASO Detection in context once it is public (I can discuss it on the call, but do not want to write anything down for now)}












